Sum-capacity of Interference Channels with a Local View: Impact of Distributed Decisions

Due to the large size of wireless networks, it is often impractical for nodes to track changes in the complete network state. As a result, nodes have to make distributed decisions about their transmission and reception parameters based on their local view of the network. In this paper, we characterize the impact of distributed decisions on the global network performance in terms of achievable sum-rates. We first formalize the concept of local view by proposing a protocol abstraction using the concept of local message passing. In the proposed protocol, nodes forward information about the network state to other neighboring nodes, thereby allowing network state information to trickle to all the nodes. The protocol proceeds in rounds, where all transmitters send a message followed by a message by all receivers. The number of rounds then provides a natural metric to quantify the extent of local information at each node. We next study three network connectivities, Z-channel, a three-user double Z-channel and a reduced-parametrization $K$-user stacked Z-channel. In each case, we characterize achievable sum-rate with partial message passing leading to three main results. First, in many cases, nodes can make distributed decisions with only local information about the network and can still achieve the same sum-capacity as can be attained with global information irrespective of the actual channel gains. Second, for the case of three-user double Z-channel, we show that universal optimality is not achievable if the per node information is below a threshold. Third, using reduced parametrization $K$-user channel, we show that very few protocol rounds are needed for the case of very weak or very strong interference.

==> 7-conclusions.tex <==
\section{Conclusions}

Almost all networks operate with partial network information at different nodes, requiring nodes to make distributed decisions. While a rich literature exists on design of network protocols and their analysis, there is no prior work to understand the impact of distributed decisions on Shannon-theoretic capacity region. In this paper, we laid foundation to characterize partial network information and studied the impact in several network connectivities. Seeking universal optimality, where local decisions with certain side information are always globally optimal, we discovered that there appears to be a critical minimum information required for the network to allow globally optimal decisions. Our current approach is compound capacity based and our next step is to understand impact of partial information on fading interference channels.

%Message passing for a class of interference channels where each transmitter is one hop away from its receiver has been considered in this paper. We explore an algorithm for message-passing  which allows nodes to incrementally learn the network state. With the intermediate knowledge at the transmitter, they decide on the rate point and the strategy based on the existing knowledge. We find the sum-rates for a deterministic and Gaussian double Z-channel which can be achieved after one and a half, and two and a half rounds. Two and a half rounds are sufficient for transmitters to converge to a rate pair on the maximum sum-rate point in the capacity region for the deterministic model, in a distributed fashion. For a Gaussian model, two and a half rounds are sufficient for transmitters to converge to a rate pair whose sum rate is within 4 bits of the sum capacity in a distributed fashion. For certain parameter values, one and a half rounds are also sufficient to achieve the maximal sum-rate. We also define the notion of universally optimal strategy to denote a strategy that is optimal with partial information and find that there does not exist any universally optimal strategy for deterministic double Z-channel with 1.5 rounds of information. Further, symmetric $K$-user one-sided interference channel where $K$ is unknown is considered. The sum capacity for varying values of the channel gains is explored and it is found that this side-information of symmetry reduces needed message passing rounds to achieve the optimal sum capacity significantly in many cases.

